TellusLoom: Weaving Knowledge into Synthetic Worlds for Dense Prediction in Remote Sensing

Dense prediction in very-high-resolution (VHR) optical remote sensing requires costly manual annotations. Synthetic worlds provide scalable supervision, yet indiscriminate 3D asset and rendering complexity is costly and does not alone guarantee transfer to real imagery. We introduce TellusLoom, a knowledge-driven framework that encodes domain knowledge as executable world rules--priors, conditional dependencies, and constraints--across five coupled dimensions of world design. Two independent generators, the asset-rich TellusLoom-Detailed (TL-D) and the lightweight, CPU-only TellusLoom-Mini (TL-M), generate imagery with aligned labels for land-cover mapping, height estimation, building change detection, and building instance segmentation, at approximately 9.7x and 382x the generation throughput of SynRS3D, respectively. Their equal mixture (TL-Mix) improves synthetic-only transfer over SynRS3D by 9.15 mIoU in land-cover mapping, reduces height mean absolute error (MAE) by 1.252 m, improves building-change F1 by 10.99 points, and reaches 37.11 mask AP for building instances; it also improves downstream performance when real training labels are scarce. Beyond a fixed dataset, the throughput of TL-M turns procedural generation into an extensible and controllable platform. Extensibility: when new object categories are requested, lightweight category cards generate supervision on demand within hours, without manual 3D modeling or real labels; specialists for 15 such categories exceed the per-category best training-free open-vocabulary method by 13.0 mean IoU on iSAID. Controllability: rule ablations and targeted interventions show how executable rules, texture strength, scene-composition coverage, and observation geometry shape transfer. Together, these findings favor preserving task-relevant world structure over indiscriminately scaling asset complexity. Code and datasets will be released.

==> supp_contents.tex <==
\makeatletter
\newcommand\SuppTocStart{}%
\newcommand\SuppContentsSetup{%
  \def\cvprsect##1{\cvprsection[##1]{\texorpdfstring{\hskip -1em.~}{}##1}}%
  \def\cvprsubsect##1{\cvprsubsection[##1]{\texorpdfstring{\hskip -1em.~}{}##1}}%
  \addtocontents{toc}{\protect\SuppTocStart}%
  \pdfbookmark[0]{Supplementary Material}{supp.material}}
\newcommand\printsuppcontents{%
  \section*{Supplementary contents}%
  \begingroup
    \setcounter{tocdepth}{2}%
    \renewcommand\@pnumwidth{2.2em}%
    \renewcommand\@tocrmarg{2.55em plus 1fil}%
    \hypersetup{linktoc=all}%
    \let\Supp@contentsline\contentsline
    \def\contentsline##1##2##3##4{}%
    \def\SuppTocStart{\let\contentsline\Supp@contentsline}%
    \@starttoc{toc}%
  \endgroup
  \par\medskip}%
\newcount\Supp@seccount
\newtoks\Supp@lefttoks
\newtoks\Supp@righttoks
\def\Supp@split{5}%
\def\Supp@sectionword{section}
\def\Supp@collect#1#2#3#4{%
  \def\Supp@kind{#1}%
  \ifx\Supp@kind\Supp@sectionword \global\advance\Supp@seccount by 1 \fi
  \ifnum\Supp@seccount<\Supp@split\relax
    \global\Supp@lefttoks\expandafter{\the\Supp@lefttoks\Supp@contentsline{#1}{#2}{#3}{#4}}%
  \else
    \global\Supp@righttoks\expandafter{\the\Supp@righttoks\Supp@contentsline{#1}{#2}{#3}{#4}}%
  \fi}
\newcommand\SuppTitleWithContents{%
  \newpage
  \twocolumn[{%
    \centering
    {\Large \textbf{\thetitle}\\ \vspace{0.5em}Supplementary Material\\ \vspace{1.0em}}%
    \begingroup
      \normalsize\normalfont\raggedright
      {\large\bfseries Supplementary contents\par}\vspace{6pt}%
      \setcounter{tocdepth}{2}%
      \renewcommand\@pnumwidth{2.2em}%
      \renewcommand\@tocrmarg{2.55em plus 1fil}%
      \hypersetup{linktoc=all}%
      \let\Supp@contentsline\contentsline
      \global\Supp@seccount=0 \global\Supp@lefttoks{}\global\Supp@righttoks{}%
      \def\contentsline##1##2##3##4{}%
      \def\SuppTocStart{\let\contentsline\Supp@collect}%
      \@starttoc{toc}%
      \noindent
      \begin{minipage}[t]{\columnwidth}\the\Supp@lefttoks\end{minipage}\hfill
      \begin{minipage}[t]{\columnwidth}\the\Supp@righttoks\end{minipage}\par
    \endgroup
    \vspace{16pt}%
  }]}
\makeatother

